Virtual crossings and a filtration of the triply graded homology of a link diagram

A filtration of Soergel bimodules by virtual crossing bimodules extends to Rouquier's complexes associated with braid words. We show that these complexes are invariant up to filtered homotopy with respect to the second Reidemeister move, and the filtration of the triply graded link diagram homology, constructed by Khovanov through the application of the Hochschild homology, is invariant under Markov moves. We also prove that the homotopy equivalence of the complexes of braid words related by the third Reidemeister move violates filtration by at most two units.

==> defs/locdef.tex <==
\def\xI{I}
\def\xJ{J}
\def\xK{K}
\def\xL{L}
\def\xM{M}
\def\xN{N}

\def\xrI{ \bar{\xI} }
\def\xrJ{ \bar{\xJ} }
\def\xrK{ \bar{\xK} }
\def\xrL{ \bar{\xL} }
\def\xrM{ \bar{\xM} }
\def\xrN{ \bar{\xN} }

%\def\xi{ i }
\def\xj{ j }
\def\xk{ k }
\def\xl{ l }
\def\xm{ m }
\def\xn{ n }

\def\xri{ \bar{\xi} }
\def\xrj{ \bar{\xj} }
\def\xrk{ \bar{\xk} }
\def\xrl{ \bar{\xl} }
\def\xrm{ \bar{\xm} }
\def\xrn{ \bar{\xn} }

\def\xip{ \xi\p }
\def\xjp{ \xj\p }
\def\xkp{ \xk\p }
\def\xlp{ \xl\p }
\def\xmp{ \xm\p }
\def\xnp{ \xn\p }

\def\xrip{ \xri\p }
\def\xrjp{ \xrj\p }
\def\xrkp{ \xrk\p }
\def\xrlp{ \xrl\p }
\def\xrmp{ \xrm\p }
\def\xrnp{ \xrn\p }

\def\xA{ A }
\def\xB{ B }
\def\xC{ C }
\def\xD{ D }
\def\xE{ E }
\def\xF{ F }

\def\xrA{ \bar{\xA} }
\def\xrB{ \bar{\xB} }
\def\xrC{ \bar{\xC} }
\def\xrD{ \bar{\xD} }
\def\xrE{ \bar{\xE} }
\def\xrF{ \bar{\xF} }

\def\xa{ a }
\def\xb{ b }
\def\xc{ c }
\def\xd{ d }
\def\xe{ e }
\def\xf{ f }

\def\xra{ \bar{\xa} }
\def\xrb{ \bar{\xb} }
\def\xrc{ \bar{\xc} }
\def\xrd{ \bar{\xd} }
\def\xre{ \bar{\xe} }
\def\xrf{ \bar{\xf} }

\def\xmu{ \mu }
\def\xnu{ \nu }
\def\xrho{ \rho }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\BRST{BRST}
\def\Ec{Inter-fiber connection}
\def\aEc{a \Ec}
\def\thEc{the \Ec}

\def\Bth{B-theory}

\def\Fc{fibration connection}

\def\hK{hyper-K\"{a}hler}
\def\pbk{pull-back}

\def\LC{Levi-Civita}
\def\LCc{\LC\ connection}

\def\cvdr{covariant derivative}
\def\cvdrs{\cvdr s}


\def\yX{ X }
\def\yY{ Y }
\def\yZ{ Z }
\def\yW{ W }

\def\yN{ n }
\def\yM{ m }

\def\yeta{ \eta }
\def\ychi{ \chi }

\def\yetav#1{ \yeta^{\bar{#1}} }
\def\yetaI{ \yetav{\xI} }
\def\yetaJ{ \yetav{\xJ} }
\def\yetai{ \yetav{\xi} }
\def\yetaj{ \yetav{\xj} }

\def\ychiv#1#2{ \ychi_{#1}^{#2} }
\def\ychim#1{ \ychiv{\xmu}{#1} }
\def\ychin#1{ \ychiv{\xnu}{#1} }
\def\ychir#1{ \ychiv{\xrho}{#1} }

\def\ychimI{ \ychim{\xI} }
\def\ychimi{ \ychim{\xi} }

\def\lrbcb#1{ \big( #1 \big) }

\def\LVbr#1#2#3{ [\zV_{#1},#2]^{#3} }
\def\LVdr{ \mathrm{L}_{\zV} }
\def\LVdrv#1{ \lrbcb{ \LVdr #1} }


\def\xee{\begin{equation}}
\def\yee{\end{equation}}


\def\mtg{ \mathrm{g} }
\def\mtgv#1#2{ \mtg_{#1\bar{#2}} }
\def\mtgij{ \mtgv{\xi}{\xj} }
\def\mtgIJ{ \mtgv{\xI}{\xJ} }
\def\mtgab{ \mtgv{\xa}{\xb} }

\def\mtgiv#1#2{ \mtg^{\bar{#1}#2} }

\def\xCG{ \Gamma }
\def\CGv#1#2#3{ \xCG^{#1}_{#2#3} }
\def\CGijk{ \CGv{\xi}{\xj}{\xk} }

\def\xCg{ \gamma }
\def\Cgv#1#2#3{ \xCg^{#1}_{#2#3} }
\def\Cgabc{ \Cgv{\xa}{\xb}{\xc} }

\def\yCg{ \gamma }
\def\yCgv#1#2#3{ \yCg^{#1}_{#2#3} }
\def\yCgijk{ \yCgv{\xi}{\xj}{\xk} }

\def\RR{ \mathrm{R} }
\def\RRv#1#2#3#4{ \RR^{#1}_{#2#3\bar{#4}}}
\def\RRJKLM{ \RRv{\xJ}{\xK}{\xL}{\xM} }
\def\RRabcd{ \RRv{\xa}{\xb}{\xc}{\xd} }

\def\cRR{ \mathcal{R} }
\def\cRRv#1#2#3#4{ \cRR^{#1}_{#2#3\bar{#4}}}
\def\cRRABCD{ \cRRv{\xA}{\xB}{\xC}{\xD} }

\def\ER{ \mathrm{R} }
\def\ERv#1#2#3{ \ER^{#1}_{#2\bar{#3}} }
\def\ERaij{ \ERv{\xa}{\xi}{\xj} }

\def\ERsv#1#2#3{ \ER^{#1}_{#2#3} }
\def\ERbv#1#2#3{ \ER^{\bar{#1}}_{\bar{#2}#3} }
\def\ERsbv#1#2#3{ \ER^{\bar{#1}}_{\bar{#2}\bar{#3}} }

\def\ERsaij{ \ERsv{\xa}{\xi}{\xj} }

\def\ERbaij{ \ERbv{\xa}{\xi}{\xj} }

\def\delv#1{ \del_{#1}\, }
\def\delm{ \delv{\xmu} }
\def\deln{ \delv{\xnu} }
\def\delr{ \delv{\xrho} }
\def\delth{ \delv{3} }

\def\nblv#1{ \nabla_{#1} }
\def\nblmu{ \nblv{\xmu} }

\def\tnbl{ \tilde{\nabla} }
\def\tnblv#1{ \tnbl_{#1} }

\def\xpar{ \parallel }
\def\xprp{ \perp }

\def\nblpar{ \nabla^\xpar }
\def\nblprp{ \nabla^\xprp }
\def\nblparv#1{ \nblpar_{#1} }
\def\nblprpv#1{ \nblprp_{#1} }
\def\nblpara{ \nblparv{\xa} }
\def\nblprpi{ \nblprpv{\xi} }

\def\mrQ{ \mathrm{Q} }
\def\dltQ{ \delta_{\mrQ} }
\def\dltQb#1{ \dltQ\lrbcb{#1} }

\def\xve{ v }
\def\xom{ \omega }
\def\vfv#1{ \xve^{#1} }
\def\vfa{ \vfv{\xa} }
\def\omfv#1{ \xom_{#1} }

\def\vfa{ \vfv{\xa} }
\def\vfb{ \vfv{\xb} }
\def\vfc{ \vfv{\xc} }
\def\vfi{ \vfv{\xi} }

\def\vpar{ \xve_{\xpar} }
\def\vprp{ \xve_{\xprp} }

\def\vparv#1{ \vpar^{#1} }
\def\vprpv#1{ \vprp^{#1} }

\def\vpara{ \vparv{\xa} }
\def\vparb{ \vparv{\xb} }
\def\vparc{ \vparv{\xc} }
\def\vprpi{ \vprpv{\xi} }

\def\xwe{ w }
\def\wfv#1{ \xwe^{#1} }
\def\wfA{ \wfv{\xA} }

\def\wpar{ \xwe_{\xpar} }
\def\wprp{ \xwe_{\xprp} }
\def\wparv#1{ \wpar^{#1} }
\def\wprpv#1{ \wprp^{#1} }

\def\wpara{ \wparv{\xa} }
\def\wprpi{ \wprpv{\xi} }

\def\xphi{ \phi }
\def\xphiv#1{ \phi^{#1} }
\def\xphiI{ \xphiv{\xI} }
\def\xphirJ{ \xphiv{\xrJ} }
\def\xphia{ \xphiv{\xa} }
\def\xphirb{ \xphiv{\xrb} }
\def\xphij{ \xphiv{\xj} }
\def\xphirj{ \xphiv{\xrj} }

\def\yN{ n }
\def\yM{ m }

\def\zV{ V }
\def\zVv#1#2{ \zV^{#1}_{#2} }
\def\zVai{ \zVv{\xa}{\xi} }

\def\zVrv#1#2{ \zVv{\bar{#1}}{\bar{#2}} }
\def\zVrai{ \zVrv{\xa}{\xi} }

\def\zVbv#1#2{ \zV^{\bar{#1}}_{\bar{#2}} }


\def\bulk{ \mathrm{bulk} }
\def\bndr{ \mathrm{bndr} }
\def\Lgr{ \mathcal{L} }
\def\Lgrv#1{ \Lgr_{#1} }
\def\Lgro{ \Lgrv{1} }
\def\Lgrt{ \Lgrv{2} }

\def\Lgrb{ \Lgr^\bulk }
\def\Lgrbv#1{ \Lgrb_{#1} }
\def\Lgrbo{ \Lgrbv{1} }
\def\Lgrbt{ \Lgrbv{2} }

\def\Lgrn{ \Lgr^\bndr }
\def\Lgrnv#1{ \Lgrn_{#1} }
\def\Lgrno{ \Lgrnv{1} }
\def\Lgrnt{ \Lgrnv{2} }


\def\Vgr{ \mathcal{V} }
\def\Vgrv#1{ \Vgr_{#1} }
\def\Vgro{ \Vgrv{1} }
\def\Vgrt{ \Vgrv{2} }

\def\Vgrb{ \Vgr^\bulk }
\def\Vgrbv#1{ \Vgrb_{#1} }
\def\Vgrbo{ \Vgrbv{1} }
\def\Vgrbt{ \Vgrbv{2} }

\def\Vgrn{ \Vgr^\bndr }
\def\Vgrnv#1{ \Vgrn_{#1} }
\def\Vgrno{ \Vgrnv{1} }
\def\Vgrnt{ \Vgrnv{2} }

\def\Tng{ \mathrm{T} }
\def\Tngv#1{ \Tng^{#1} }
\def\Tngpar{ \Tngv{\xpar} }
\def\Tngprp{ \Tngv{\xprp} }


\def\cA{ \mathcal{A} }
\def\cAv#1#2#3{ \cA^{#1}_{#2#3} }
\def\cAABC{ \cAv{\xA}{\xB}{\xC} }
\def\tcA{ \tilde{\cA} }
\def\tcAv#1#2#3{ \tcA^{#1}_{#2#3} }
\def\tcAABC{ \tcAv{\xA}{\xB}{\xC} }

\def\trT{ \mathcal{T} }
\def\trTv#1#2#3{ \trT^{#1}_{#2#3} }
\def\trTABC{ \trTv{\xA}{\xB}{\xC} }
\def\trTajk{ \trTv{\xa}{\xj}{\xk} }

\def\yveps{ \varepsilon }
\def\yvepsmnr{ \yveps_{\xmu\xnu\xrho} }
\def\yvepsmn{ \yveps_{\xmu\xnu} }
\def\yeps{ \epsilon }
\def\yepsv#1#2{ \yeps_{#1#2} }
\def\yepsIJ{ \yepsv{\xI}{\xJ} }
\def\yepsKJ{ \yepsv{\xK}{\xJ} }

\def\yepsiv#1#2{ \yeps^{#1#2} }

\def\mpi{ \pi }
\def\mpiv#1{ \mpi_{#1} }
\def\mpiphiI{ \mpiv{\xphiI} }
\def\mpiphirJ{ \mpiv{ \xphirJ} }


\def\wEta{ H }
\def\wEtav#1{ \wEta^{\bar{#1}} }
\def\wEtaA{ \wEtav{\xA} }

\def\weta{ \eta }
\def\wetav#1{ \weta^{\bar{#1}} }
\def\wetaa{ \wetav{\xa} }
\def\wetab{ \wetav{\xb} }

\def\wRho{ P }
\def\wRhov#1#2{ \wRho_{#1}^{#2} }
\def\wRhomA{ \wRhov{\xmu}{\xA} }

\def\wrho{ \rho }
\def\wrhov#1#2{ \wrho_{#1}^{#2} }
\def\wrhoma{ \wrhov{\xmu}{\xa} }

\def\wtheta{ \theta }
\def\wthetav#1{ \theta_{#1} }
\def\wthetaa{ \wthetav{\xa} }

\def\wF{ F }
\def\wFv#1{ \wF^{#1} }
\def\wFA{ \wFv{\xA} }

\def\wf{ f }
\def\wfnv#1{ \wf^{#1} }
\def\wfa{ \wfnv{\xa} }

